A Neural Passage Model for Ad-hoc Document Retrieval

Traditional statistical retrieval models often treat each document as a whole. In many cases, however, a document is relevant to a query only because a small part of it contain the targeted information. In this work, we propose a neural passage model (NPM) that uses passage-level information to improve the performance of ad-hoc retrieval. Instead of using a single window to extract passages, our model automatically learns to weight passages with different granularities in the training process. We show that the passage-based document ranking paradigm from previous studies can be directly derived from our neural framework. Also, our experiments on a TREC collection showed that the NPM can significantly outperform the existing passage-based retrieval models.

==> model_separate_two_model.tex <==
%!TEX root=SIGIR17Short-PassageRetrieval.tex
\section{Passage-based Document Ranking}\label{sec:passage_model}

Passage-based retrieval models use passages as representatives for each document and rank documents according to their passage scores.
As discussed in Section~\ref{sec:related}, most passage-based retrieval models extracted passages with a fixed-length window and the state-of-the-art method computes a passage score by applying the language modeling approach on each passage~\cite{liu2002passage,bendersky2008utilizing}.
Specifically, given a query $q$ and a passage $g$, the score of $g$ is the maximum log likelihood of observing $q$ given $g$'s unigram language model as
\begin{equation}
\log P(q|g) = \sum_{t \in q}\log((1-\lambda_c)\frac{tf_{t,g}}{n} + \lambda_c\frac{cf_t}{|C|})
\label{equ:language_model}
\end{equation}
where $tf_{t,g}$ is the count of $t$ in $g$, $cf_t$ is the corpus frequency of $t$, $|C|$ is the length of the corpus and $\lambda_c$ is a smoothing parameter.

Assuming that passages can serve as proxies of documents~\cite{bendersky2008utilizing}, the ranking score of a document $d$ under that passage-based document ranking framework should be 
\begin{equation}
Score(q, d) = \log\sum_{g \in d}P(g|d)\cdot P(q|g)
\end{equation}
Intuitively, $P(g|d)$ could be an uniform distribution as all passages are extracted following the same methodology.
However, averaging passage scores produces poor retrieval performance in practice and the state-of-the-art models prefer a winner-take-all strategy that only uses the best passage to compute document scores~\cite{liu2002passage,bendersky2008utilizing}:  
\begin{equation}
Score(q, d) = \max_{g \in d} \log P(q|g)
\label{equ:max}
\end{equation}

%When $\{g_i|i\in \left[0,\lfloor \frac{n_d}{\tau} \rfloor \right]\}$ is generated with the same convolution filter, it is intuitive to define a uniform distribution for $P(g_i|d)$. 
%However, using the average of passage scores contradicts our motivation in Section~\ref{sec:introduction} and produces poor retrieval performance \cite{liu2002passage,bendersky2008utilizing}. 
%Instead, a winner-take-all strategy that only uses the best passage score is more popular in practice \cite{callan1994passage,kaszkiel2001effective,wilkinson1994effective,liu2002passage,bendersky2008utilizing}:
%\begin{equation}
%Score(q, d) = \max_{g_i} Score(q,g_i)
%\end{equation}
%In our proposed neural network framework, this strategy is implemented with a max-pooling layer over the convolution layer on the matching matrix $M(q,d)$.

%probability of $q$ given the unigram language model of $g$ ($M_g$)


\section{Neural Passage Model}
\label{sec:neural_model}

In this section, we describe the structure of the neural passage retrieval model. 
%Passage-based retrieval models use passages as representatives for each document and rank documents according to their passage scores.    
The extraction of window-based passages in our model is actually a convolution process on the matching matrix of query-document terms, and the passage language model used by prior work can be viewed as a logarithm kernel with mean and max pooling in the convolution layer.
Further, to aggregate information from different sizes of passages, we propose a fusion network that considers both document homogeneity and query characteristics.
%we propose a fusion network that aggregates information from different sizes of passages to form the final ranking scores.  
%The overall structure of the neural passage model is shown in Figure~\ref{fig:npm}.

\begin{figure}
	\centering
	\includegraphics[width=3.6in]{./figure/model_structure.pdf}
	\caption{The structure of the neural passage model. $n_d$, $n_q$ are the length of document $d$ and query $q$; $M(q,d)$ is the matching matrix; $m$, $\tau$, $g_i$, $K(q,g_i)$ are the window size, stride size, $i$th passage and corresponding output of convolution kernel $K$; $\vec{r}(q,d)$ is the passage scores with different granularities; $\vec{h}(q,d)$ denotes query/document features and $f(q,d)$ is the final ranking score for $q$ and $d$ (Equation~\ref{equ:fusion}).}
	\label{fig:npm}
\end{figure}

%\subsection{Convolution and Passage Extraction}
\textbf{\textit{Passage Extraction with a Convolution Layer}}.\label{sec:convolution}
%Window-based passage extraction is widely used for retrieval tasks \cite{zobel1995efficient,liu2002passage,bendersky2008utilizing}. 
Given a fixed length window, window-based passages are extracted by sliding the window along the document with fixed step size. 
Formally, given a document $d$ with length $n_d$, the set of extracted passages $G(d)$ with window size $m$ and step size $\tau$ is $G(d) = \{ g_i | i \in \left[ 0, \lfloor \frac{n_d}{\tau} \rfloor \right]  \}$
%\begin{equation}
%G(d) = \{ g_i | i \in \left[ 0, \lfloor \frac{n_d}{\tau} \rfloor \right]  \}
%\end{equation}
where $g_i$ represents the $i$th passage starting from the $i\cdot\tau$th term in $d$ with size $m$. 
%When $\tau$ is smaller than $m$, extracted window-based passages have overlaps with their neighbors.
%\begin{figure}
%	\centering
%	\includegraphics[width=3in]{./figure/convolution.pdf}
%	\caption{Passage extraction as a convolution process on the matching matrix of query $q$ and document $d$ ($M(q,d)$) with filter size $m$, stride $\tau$ and kernel function $K$.}
%	\label{fig:convolution}
%\end{figure}
 %(either binary matching or matching with word embeddings). 
%If $q$ has $n_q$ terms and $d$ has $n_d$ terms, then $M(q,d)$ is a $(n_q, n_d)$ dimensional matrix in which the cell $M(q,d)_{i,j}$ represents the matching score between the $i$th term in $q$ and the $j$th term in $d$. 
%Let $M(q,d)$ be the matching matrix of terms in query $q$ and document $d$, and $n_q$ be the length of $q$, then $M(q,d)$ is a $\mathbb{R}^{n_q\times n_d}$ dimensional matrix in which $M(q,d)_{i,j}$ represents the matching of the $i$th term in $q$ and the $j$th term in $d$. 
Let $n_q$ be the length of query $q$, then the matching of terms in $q$ and $d$ is a matrix  $M(q,d) \in \mathbb{R}^{n_q\times n_d}$ in which $M(q,d)_{i,j}$ represents the matching between the $i$th term in $q$ and the $j$th term in $d$.
%In the simplest case, the matching score is a binary variable (1 if the two terms are same and 0 if they are not), but it could also be other value such as the cosine similarity between the term's embedding representations. 
The matching of two terms can either be scalar (i.e. the cosine similarity between word embeddings) or binary (1 if the two terms are same and 0 if they are not).
%Let $K(q,g_i)$ be the score of passage $g_i$ given $q$, then the sliding window used in window-based passage approach can be  a convolution filter with size $m$, stride $\tau$ and kernel function $K$ over $M(q,d)$, which is shown in the left hand side of Figure~\ref{fig:npm}. 
Let $K(q,g_i)$ be the score of $g_i$ given $q$, then the extraction of window-based passages can be achieved with a convolution filter with size $m$, stride $\tau$ and kernel $K$ over $M(q,d)$.
With multiple filters, we extract passages with different granularities for further processing (the left-hand side of Figure~\ref{fig:npm}). 
%The extraction of window-based passages is actually a convolution process.

\iffalse
%The bridge between window-based passages and convolution is important because convolution is a standard process in neural networks. 
%From this perspective, the passage extraction of previous passage-based retrieval models~\cite{liu2002passage,bendersky2008utilizing} can be viewed a convolution layer with fixed filters in our neural network framework.
%By formulating a convolution layer, we can derive previous passage-based retrieval models as special cases in our neural network framework, which will be discussed later in this section.
\fi


%\subsection{Language Model as a Logarithm Kernel}
\textbf{\textit{Language Modeling as a Logarithm Kernel}}.\label{sec:language_model}
%Language modeling refers to the problem of estimating the likelihood of observing certain piece of text given a particular language distribution. 
%A standard language modeling approach in IR~\cite{ponte1998language} ranks documents according to the probability of observing the query given the document language model.
%More specifically, the probability of query $q$ given document $d$ in a unigram language model is $P(q|d) = \prod_{t \in q}P(t | M_d)$
%\begin{equation}
%P(q|d) = \prod_{t \in q}P(t | M_d)
%\end{equation}
%where $t$ is the term in $q$ and $M_d$ is the language model of $d$.
%A common paradigm for estimating $P(t | M_d)$ is using the maximum likelihood estimation with corpus-based language smoothing, so the ranking scores of documents can be formulated as
%\begin{equation}
%P(t|M_d) = (1-\lambda_c)\frac{tf(t,d)}{n_d} + \lambda_c\frac{cf_t}{|C|}
%\end{equation} 
%\begin{equation}
%Score(q, d) = \sum_{t \in q}\log((1-\lambda_c)\frac{tf_t}{n} + \lambda_c\frac{cf_t}{|C|})
%\label{equ:language_model}
%\end{equation}
%where $tf(t,d)$ is the count of $t$ in $d$, $cf_t$ is the corpus frequency of $t$, $|C|$ is the length of the corpus and $\lambda_c$ is a smoothing parameter. %. range from 0 to 1.
%where $tf(t,d)$ is the count of $t$ in $d$, $n_d$ is the length of $d$, $cf_t$ is the corpus frequency of $t$, $|C|$ is the length of the corpus and $\lambda_c$ is a smoothing parameter range from 0 to 1.
%Under this framework, documents are ranked with the log likelihood of $P(q|d)$ as 
Previous passage-based retrieval models computes passage scores by estimating the log likelihood of observing the query given the passage language model.
In fact, the score function of the language modeling approach in Equation~\ref{equ:language_model} can be viewed as a logarithm activation function over the linear projection of $M(q,g)$. 
%Let $M(t,g_i)$ be a matching matrix between term $t$ and $g_i$ with shape $(1,m,1)$, where the last dimension represents the matching score between $t$ and a term in $g_i$ (which is 1 when we only consider binary matching).
%Then the passage language model can be formulated as 
Let $M(t,g_i)$ be the binary matching matrix for term $t$ and $g_i$ with shape $(1,m)$, then the passage language model score can be formulated as
\begin{equation}
Score(q, g_i) \sim \sum_{t \in q}\log(W\cdot M(t,g_i)  + b_t)
\label{equ:kernel}
\end{equation}
where $W$ is a constant matrix with elements equal to 1, and $b_t$ is a bias term equal to $\frac{\lambda_c \cdot m \cdot  cf_t}{(1-\lambda_c) |C|}$.
Also, the passage-based document ranking strategy in Equation~\ref{equ:max} can be viewed as a max-pooling layer over the mean-pooling of convolution outputs (the middle part of Figure~\ref{fig:npm}).
%, which is a common structure widely used in neural networks.
The computation of passage language scores is actually a logarithm convolution kernel with mean pooling over the columns of $M(q,g)$ and max pooling over the rows of mean-pooling's outputs.
Up to this point, we successfully unified the passage-based document ranking with a convolution neural network framework.% framework without the loss of generality.
%The language modeling approach can be viewed as a logarithm convolution kernel with fixed parameters.
%Considering the relationship between window-based passage extraction and convolution process, the construction of passage language models is actually a convolution layer with logarithm kernel function.

\iffalse
%To incorporate more complicated matching signals like the matching of word embeddings (e.g. word2vec~\cite{mikolov2013efficient}), one could use high dimensional matching scores for each cell in $M(t, g_i)$. 
%For example, we could discretize the cosine similarity between word embeddings of two terms into 10 bins and use a 10 dimensional vector to represent the matching score of these two terms. 
%However, using a matching matrix with high dimensional matching scores would significantly increase the number of model parameters and usually requires more data to train.
%Due to the limited size of training data on TREC collections, we did not observe significant improvement on retrieval performance by replacing binary matching with the matching of word vectors produced by word2vec. 
\fi


\textbf{\textit{Aggregating Passage Models with a Fusion Network}}.
Bendersky and Kurland observed that the usefulness of passage level information varies on different documents\cite{bendersky2008utilizing}. 
To consider document characteristics, they proposed to combine the passage models with document models using document homogeneity scores:
\begin{equation}
Score(q, d) = h^{[M]}(d)P(q|d) + (1 - h^{[M]}(d))\max_{g \in d}P(q|g)
\label{equ:max}
\end{equation}
where $h^{[M]}(d)$ could be the length-based homogeneity $h^{\left[ length \right] }$, the entropy-based homogeneity $h^{\left[ ent \right] }$, the inter-passage homogeneity $h^{\left[ intPsg \right] }$ or the doc-passage homogeneity $h^{\left[ docPsg \right] }$:
\begin{equation}
\begin{split}
h^{\left[ length \right]}(d)  &= 1 - \frac{\log n_d - \min_{d_i \in C}\log n_{d_i}}{\max_{d_i \in C}\log n_{d_i} - \min_{d_i \in C}\log n_{d_i}}\\
h^{\left[ ent \right]}(d)  &= 1 + \frac{\sum_{t'\in d}P(t' |d)\log (P(t' |d))}{\log n_d}\\
h^{\left[ intPsg \right]}  &= \frac{2}{\lceil \frac{n_d}{\tau} \rceil(\lceil \frac{n_d}{\tau} \rceil -1)}\sum_{i < j;g_i, g_j \in d}\cos(g_i,g_j)\\
h^{\left[ docPsg \right]}  &= \frac{1}{\lceil \frac{n_d}{\tau} \rceil}\sum_{g_i \in d}\cos(d,g_i)
\end{split}
\label{equ:homogeneity}
\end{equation}
In Equation~\ref{equ:homogeneity}, $C$ is the corpus and $\cos(d, g_i)$ is the cosine similarity between the tf.idf vector of $d$ and $g_i$.

Inspired by the design of homogeneity scores and previous studies on query performance prediction~\cite{zhao2008effective}, we propose a fusion network that aggregates passage scores from different granularities according to both document properties and query characteristics. 
Besides the document homogeneity features, we extract features for queries and concatenate them together to from a fusion feature vector $\vec{h}(q,d)$.
We use three types of query quality features and one list-based feature, which is the average scores of top 2,000 documents retrieved by the language modeling approach.
The query quality features are: 
\begin{equation}
\begin{split}
IDF_t &= \frac{\log\frac{|D|+0.5}{D_t}}{|D|+1}, ~~~~ICF_t = \log\frac{cf_t}{|C|} \\
SCQ_t &= (1 + \log(cf_t))\log(1 + \frac{|D|}{D_t}) \\
\end{split}
\label{equ:query_features}
\end{equation}
where $D_t$ is the document frequency of term $t$ and $|D|$ is the number of documents in the whole collection. 
For each feature, we computed its sum, standard deviation, maximum/minimum, maximum, arithmetic mean, geometric mean, harmonic mean and coefficient of variation for all query terms.
Suppose that we have $\alpha$ convolution filters, $\beta$ fusion features and let $\vec{r}(q,d) \in \mathbb{R}^\alpha$ be a vector where each dimension denotes a score from a passage model with one filter size, the final ranking score of $d$ is computed as 
\begin{equation}
\begin{split}
Score(q,d) = f(q,d) &= \tanh(\vec{r}(q,d)^T\cdot \phi(\vec{h}(q,d))  + b_R) \\
\phi(\vec{h}(q,d))_i &= \frac{\exp (\vec{W_R^i}\cdot \vec{h}(q,d))}{\sum_{j=1}^{\alpha}\exp (\vec{W_R^j}\cdot \vec{h}(q,d))}
\end{split}
\label{equ:fusion}
\end{equation} 
where $W_R \in \mathbb{R}^{\alpha \times \beta}$ and $b_R\in \mathbb{R}$ are parameters learned in the training process.
We design function $\phi$ as a softmax function so that $\phi(\vec{h}(q,d))_i$ is positive and sums up to 1.
Therefore, the value of $\phi(\vec{h}(q,d))_i$ can be viewed as the weight of passage scores on the $i$th dimension of $\vec{r}(q,d)$.

\textbf{\textit{Model Optimization}}.
We employ a pairwise hinge loss to train the neural passage model. Given a triple $(q,d^+,d^-)$ where $d^+$ is relevant and $d^-$ is irrelevant with respect to $q$, the loss function is formulated as:
\begin{equation}
\ell(q,d^+,d^- | \Theta) = \max(0, 1-s(q,d^+)+s(q,d^-))
\end{equation} 
where $\Theta$ represents all parameters in the model.
We apply stochastic gradient descent with mini-batches and early stopping \cite{giles2001overfitting} in the training process. 




%Plus, we add a group of list-based features by computing the same statistics over the language model scores of top 2,000 documents retrieved by the language modeling approach \cite{ponte1998language}




\iffalse
as discuss before, xxx is not vague
a better paradigm is to xxx
however, the importance of xxx depends on xxx
In previous work,xxxx
In this paper, we further extract query features and construct a fusion network to xxx
$fustion network$
the query feature we used are xxxx
we tested our models with three settings and show the results in xxx
therefore, we extracted query/document features and 



%\subsection{Model Fusion}
\textbf{\textit{Model Fusion}}\label{sec:fusion}
There are two levels of model fusion in passage-based retrieval models. The first level concerns about how to aggregate or select passages from the same sliding window. 
The second level focuses on combining the information from passages with different granularities.

%\subsubsection{Selection of Passages with Same Sizes}
As discussed in Section~\ref{sec:convolution} and \ref{sec:language_model}, each document has $\lceil \frac{n_d}{\tau}\rceil$ passages and corresponding scores $Score(q, g_i)$.
Given that these passages can serve as proxies of the document \cite{bendersky2008utilizing}, then the ranking score of $d$ given $q$ under the passage-based document ranking framework should be
\begin{equation}
Score(q, d) = \sum_{g_i}p(g_i|d)Score(q,d)
\end{equation}
When $\{g_i|i\in \left[0,\lfloor \frac{n_d}{\tau} \rfloor \right]\}$ is generated with the same convolution filter, it is intuitive to define a uniform distribution for $P(g_i|d)$. 
However, using the average of passage scores contradicts our motivation in Section~\ref{sec:introduction} and produces poor retrieval performance \cite{liu2002passage,bendersky2008utilizing}. 
Instead, a winner-take-all strategy that only uses the best passage score is more popular in practice \cite{callan1994passage,kaszkiel2001effective,wilkinson1994effective,liu2002passage,bendersky2008utilizing}:
\begin{equation}
Score(q, d) = \max_{g_i} Score(q,g_i)
\end{equation}
In our proposed neural network framework, this strategy is implemented with a max-pooling layer over the convolution layer on the matching matrix $M(q,d)$.

%\subsubsection{Aggragation of Passages with Different Granularities} 
As discussed in Section~\ref{sec:related}, there is no conclusive answer for the question of how to define the size of passages. 
Therefore, the ability to weight and aggregate multi-level passage information is essential for passage-based retrieval models.

The state-of-art passage-based retrieval model proposed by Bendersky and Kurland \cite{bendersky2008utilizing} tries to evaluate the usefulness of different passages according to the homogeneity of each document.
The basic assumption is that a document with high homogeneity should be considered as a whole while a document with low homogeneity should be cut into pieces or have short passages.
Based on this consideration, they applied four measurements to identify the homogeneity of documents.
They are length-based homogeneity $h^{\left[ length \right] }$, entropy-based homogeneity $h^{\left[ ent \right] }$, inter-passage homogeneity $h^{\left[ intPsg \right] }$ and doc-passage homogeneity $h^{\left[ docPsg \right] }$:
\begin{equation}
\begin{split}
h^{\left[ length \right]}(d)  &= 1 - \frac{\log n_d - \min_{d_i \in C}\log n_{d_i}}{\max_{d_i \in C}\log n_{d_i} - \min_{d_i \in C}\log n_{d_i}}\\
h^{\left[ ent \right]}(d)  &= 1 + \frac{\sum_{t'\in d}P(t' |d)\log (P(t' |d))}{\log n_d}\\
h^{\left[ intPsg \right]}  &= \frac{2}{\lceil \frac{n_d}{\tau} \rceil(\lceil \frac{n_d}{\tau} \rceil -1)}\sum_{i < j;g_i, g_j \in d}\cos(g_i,g_j)\\
h^{\left[ docPsg \right]}  &= \frac{1}{\lceil \frac{n_d}{\tau} \rceil}\sum_{g_i \in d}\cos(d,g_i)
\end{split}
\end{equation}
where $C$ is the corpus and $\cos(d, g_i)$ is defined as the cosine similarity between the tf.idf vector of $d$ and $g_i$.
 
To generate the final ranking score for each document, Bendersky and Kurland separately tested each type of homogeneity score as weights for passage models. 
We argue that a better option is to learn this weighting scheme automatically from the training data.
Therefore, we propose a fusion network to generate the weights for each passage model.  
Let $\vec{r}(q,d)$ be a $R$ dimensional vector with each dimension representing the score from a passage model with fixed-length filters. 
Given that $\vec{h_d}$ is a $H$ dimensional feature vector of $d$ (e.g. the homogeneity scores of $d$), the final ranking score is computed as:
\begin{equation}
f(q,d) = \tanh(\vec{r}(q,d)\cdot softmax(W_R \vec{h}_d)  + b_R)
\label{equ:fusion}
\end{equation} 
where $W_R$ is a $(R,H)$ dimensional matrix and $b_R$ is a bias term.

In addition, the flexibility of neural networks enables our neural passage model to simultaneously incorporate different fusion features without major changes in network structure. 
%Therefore, we want to explore whether query information could be another important factor that determine the weight of passage models.
One question that we want to explore is whether query information could be useful to the weighting process of passage models.
Therefore, we incorporate four types of query features into our fusion network, which are IDF-based features ($IDF_t$), ICF-based features ($ICF_t$) and collection-query similarity features ($SCQ_t$) \cite{zhao2008effective,kumaran2009reducing}:
\begin{equation}
\begin{split}
IDF_t &= \frac{\log\frac{D+0.5}{D_t}}{D+1} \\
ICF_t &= \log\frac{cf_t}{|C|} \\
SCQ_t &= (1 + \log(cf_t))\log(1 + \frac{D}{D_t})
\end{split}
\label{equ:query_features}
\end{equation}
where $D_t$ is the document frequency of term $t$ and $D$ is the number of documents in the whole collection. 
For each feature above, we computed its sum, standard deviation, maximum/minimum, maximum, arithmetic mean, geometric mean, harmonic mean and coefficient of variation for all query terms.
Plus, we add a group of list-based features by computing the same statistics over the language model scores of top 2,000 documents retrieved by the language modeling approach \cite{ponte1998language} (as shown in Equation~\ref{equ:language_model}).

%\subsection{Overall Structure and Optimization}



\textbf{\textit{Overall Structure and Optimization}}.
The overall structure of our neural passage model is shown in Figure~\ref{fig:npm}.
The input of our model is the matching matrix between query terms and document terms for query $q$ and document $d$ (as described in Section~\ref{sec:convolution}). 
It is fed into a convolution layer with multiple filters and a logarithm kernel function described in Equation~\ref{equ:kernel}.
A max-pooling layer is added at the end of convolution process to generate the ranking score $r_x(q,d)$:
\begin{equation}
\begin{split}
r_x(q,d) = \max_{g_i \in G_x}\sum_{t \in q}\log(W\cdot M(t,g_i)  + b_t)
\end{split}
\end{equation}
where $G_x$ is the set of passages generated by the $x$th filter with size $m$ and stride $\tau$
The scores $r_x(q,d)$ from different filters are further packed into a single vector $\vec{r}(q,d)$ to interact with document features through a fusion network (Equation~\ref{equ:fusion}) to generates the final ranking score $s(q,d)$.

For model training, we employ a pairwise ranking loss such as hinge loss. Given a triple $(q,d^+,d^-)$ where $d^+$ is relevant and $d^-$ is irrelevant with respect to $q$, the loss function is formulated as:
\begin{equation}
\ell(q,d^+,d^- | \Theta) = \max(0, 1-s(q,d^+)+s(q,d^-))
\end{equation} 
The $\Theta$ represents all the parameters in our neural passage model.
We apply stochastic gradient descent method with mini-batches.
We note that early stopping \cite{giles2001overfitting} is beneficial for the robustness of our model. 
\fi


